Learning Fine-grained View-Invariant Representations from Unpaired Ego-Exo Videos via Temporal Alignment

The egocentric and exocentric viewpoints of a human activity look dramatically different, yet invariant representations to link them are essential for many potential applications in robotics and augmented reality. Prior work is limited to learning view-invariant features from paired synchronized viewpoints. We relax that strong data assumption and propose to learn fine-grained action features that are invariant to the viewpoints by aligning egocentric and exocentric videos in time, even when not captured simultaneously or in the same environment. To this end, we propose AE2, a self-supervised embedding approach with two key designs: (1) an object-centric encoder that explicitly focuses on regions corresponding to hands and active objects; and (2) a contrastive-based alignment objective that leverages temporally reversed frames as negative samples. For evaluation, we establish a benchmark for fine-grained video understanding in the ego-exo context, comprising four datasets -- including an ego tennis forehand dataset we collected, along with dense per-frame labels we annotated for each dataset. On the four datasets, our AE2 method strongly outperforms prior work in a variety of fine-grained downstream tasks, both in regular and cross-view settings.

==> rebuttal.tex <==
\setcounter{page}{1}
\newpage
\renewcommand{\thetable}{R\arabic{table}}
\renewcommand{\thefigure}{R\arabic{figure}}

\begin{table}[!t]
\tablestyle{3pt}{1.3}
  \caption{Comparison of AE2 employing randomly shuffled frames versus temporally reversed frames as the negative samples on all four datasets.}
  \label{tab:results}
  \centering
  \scalebox{1.0}{
  \begin{tabular}{l|l|ccccccc}
   \thickhline
\multirow{2}{*}{\makecell[c]{Dataset}} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Classification (F1 score)} & \multicolumn{3}{c}{Frame Retrieval (mAP@10)} & Phase \\ % &Kendall's \\
& & regular & ego2exo & exo2ego & regular & ego2exo & exo2ego & Progression \\ %& Tau\\
\thickhline
\multirow{2}{*}{\makecell[c]{(A) CMU-MMAC}} & Random Shuffle & 60.61 & \best{58.63} & 54.46 & 61.66 & 57.57 & 59.61 & 0.3385 \\ % & 0.4930\\
& Temporal Reverse & \best{66.23} & 57.41 & \best{71.72} & \best{65.85} & \best{64.59} & \best{62.15} & \best{0.5109} \\ %& \best{0.6316} \\
\hline
\multirow{2}{*}{\makecell[c]{(B) H2O}} & Random Shuffle & 82.05 & 82.74 & 79.48 & 81.92 & \best{80.60} & 79.71 & 0.6659 \\ %& 0.8454 \\
& Temporal Reverse & \best{85.17}    & \best{84.73}      & \best{82.77}      & \best{84.90}  & 78.48 & \best{83.41}  & \best{0.7634} \\ % & \best{0.9062} \\    
\hline
\multirow{2}{*}{\makecell[c]{(C) Pour Liquid}}  & Random Shuffle & \best{68.13} & \best{64.96} & 58.44 & 63.48 & 62.73 & \best{60.27} & -0.0121 \\ %& \best{0.1290} \\
& Temporal Reverse & 66.56 & 57.15 & \best{65.60} & \best{65.54} & \best{65.79} & 57.35 & \best{0.1380} \\ %& 0.0934  \\

\hline
\multirow{2}{*}{\makecell[c]{(D) Tennis Forehand}} & Random Shuffle & 84.12 & \best{84.83} & 82.59 & 86.73 & 80.49 & \best{83.75} & \best{0.5304} \\ %& \best{0.6206} \\
& Temporal Reverse & \best{85.87} & 84.71  & \best{85.68} & \best{86.83} & \best{81.46} & 82.07 & 0.5060 \\ %& 0.6171 \\

\thickhline
\end{tabular}
}
\end{table}

\begin{figure}[!t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/rebuttal/combined.pdf}
  \caption{Visualization of (a) the original video sequence; (b) a randomly shuffled sequence; and (c) a temporally reversed sequence on CMU-MMAC (left) and Pour Liquid (right). The randomly shuffled sequence may still preserve the action progression order due to many similar frames in the video sequence, failing to be truly ``negative''. In contrast, temporally reversing frames results in a more distinct and suitable negative example.}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/rebuttal/neg.png}
  \caption{Visualization of a video sequence (from CMU-MMAC) exhibiting a certain amount of periodicity, where the camera wearer hits the egg to the bowl's edge twice. In the upper figure, frame-level negatives are defined based on temporal distance, leading to the possibility of two visually similar frames (marked by a red border) being misclassified as a ``negative'' pair. In contrast, the lower figure illustrates how sequence-level negatives provide a more robust solution to accomodate the temporal variations within a video. }
\end{figure}
